Selecting Relevant Features from a Multi-domain Representation for Few-shot Classification

Popular approaches for few-shot classification consist of first learning a generic data representation based on a large annotated dataset, before adapting the representation to new classes given only a few labeled samples. In this work, we propose a new strategy based on feature selection, which is both simpler and more effective than previous feature adaptation approaches. First, we obtain a multi-domain representation by training a set of semantically different feature extractors. Then, given a few-shot learning task, we use our multi-domain feature bank to automatically select the most relevant representations. We show that a simple non-parametric classifier built on top of such features produces high accuracy and generalizes to domains never seen during training, which leads to state-of-the-art results on MetaDataset and improved accuracy on mini-ImageNet.

==> ccl.tex <==
In this work we introduce a method for few-shot classification, based on selecting
relevant representation from universal representations. While being conceptually
simple, our approach sets a new state-of-the-art results in cross-domain
few-shot learning. Such results indicate that learning a set of domain specific
representation and then selecting only the relevant ones for a target task
outperforms current adaptation methods. 
